Effective Sample Size, Dimensionality, and Generalization in Covariate Shift Adaptation

In supervised learning, training and test datasets are often sampled from distinct distributions. Domain adaptation techniques are thus required. Covariate shift adaptation yields good generalization performance when domains differ only by the marginal distribution of features. Covariate shift adaptation is usually implemented using importance weighting, which may fail, according to common wisdom, due to small effective sample sizes (ESS). Previous research argues this scenario is more common in high-dimensional settings. However, how effective sample size, dimensionality, and model performance/generalization are formally related in supervised learning, considering the context of covariate shift adaptation, is still somewhat obscure in the literature. Thus, a main challenge is presenting a unified theory connecting those points. Hence, in this paper, we focus on building a unified view connecting the ESS, data dimensionality, and generalization in the context of covariate shift adaptation. Moreover, we also demonstrate how dimensionality reduction or feature selection can increase the ESS, and argue that our results support dimensionality reduction before covariate shift adaptation as a good practice.

==> methods.tex <==
\section{Variable Selection for Covariate Shift Adaptation}

 Here we propose to perform feature selection prior to covariate shift adaptation. Working with a useful subset of features enables a greater ESS and can lead to a better generalization. Right after the feature selection step, the covariate shift adaptation is carried out via importance weighting using off-the-shelf methods for density ratio estimation.
 
 The following theorem supports our idea. The theorem was adapted from \cite{stojanov2019low} to accommodate some of our particularities and make some aspects more transparent.

\begin{thm}\label{thm:suf1} 
(Adapted from \cite{stojanov2019low}) Consider a loss function $L$, the source and target joint distributions $Q_{\rvx,\ry}$ and $P_{\rvx,\ry}$, with probability density functions $q_{\rvx,\ry}$ and $p_{\rvx,\ry}$ such that $\text{support}(p_{\rvz}) \subseteq \text{support}(q_{\rvz})$. Assume we partition the original set of features in the following way $\rvx=(\rvx_1,\rvx_2)$ and that Covariate Shift assumptions are valid. Suppose there is an optimal function $h^*$ in the hypothesis class $\mathcal{H}$ that minimizes the risk assessed in the target distribution. 

Assume that (i) $q_{\ry|\rvx}(.|\vx)=q_{\ry|\rvx_1}(.|\vx_1)$ almost surely and that (ii) there is a function $\tilde{h}^*(\vx_1)$ as optimal as $h^*(\vx)$, i.e. they return the same risk at target population. We suppose the new function $\tilde{h}^*$ is in a proper hypothesis set, contained in $\mathcal{H}$, such that it maps the set of features $\rvx_1$ to the labels set. For a weighting function $w$, we have 
\begin{align}
 \E_{P_{\rvx,\ry}}\Big[ L\left(h^*(\rvx),\ry \right) \Big]=\E_{Q_{\rvx_1,\ry}} \Big[ w(\rvx_1) \cdot L(\tilde{h}^*(\rvx_1),\ry ) \Big]
\end{align}
\end{thm}


The proof can be found in the Supplementary Material. Theorem \ref{thm:suf1} states that we can potentially achieve the same optimal results working with fewer features and higher ESS if assumptions (i) and (ii) are true. Notice that condition (i) could be reformulated as $\ry \independent \rvx | \rvx_1$ and does not depend on the domain we are working with, since $p_{\ry|\rvx}=q_{\ry|\rvx}$. In other words, $\rvx_1$ is statistically sufficient for $\ry$. The condition (ii) depends on the hypothesis class and essentially tells us that there exists at least one optimal hypothesis in $\mathcal{H}$ that does not depend on $\rvx_2$. The feature selection approach we propose to be used with covariate shift adaptation relies on the sufficient dimension reduction we discuss next.

\subsection{Feature selection Via Sufficient Dimension Reduction (SDR)}

SDR is a supervised technique for dimensional reduction, while preserving relevant information and minimizing redundancies from original features to create good classifiers and regressors afterwards \cite{fukumizu2004dimensionality,suzuki2010sufficient}. Given a set of features $\rvx$ and a target variable $y$, the objective of SDR is to find a matrix $\mM \in \R^{d \times d'}$, with $d' < d$ and $\mM^\top \mM=\mI_{d'}$, such that $y \independent \rvx ~|~ \mM^\top \rvx$. That is, the representation $\mM^\top \rvx$ is sufficient for $y$. Usually, $\mM$ is assumed to be dense, and in that case, $\mM$ is estimated using variations of the gradient descent algorithm. We focus on the case where the matrix $\mM$ is sparse, and each column of it is given by zeros, except for one entry set as $1$ to create a feature selector, as it is done by \cite{fukumizu2004dimensionality}. 

An interesting way to face the problem of sufficient dimension reduction is using the concept of mutual information \cite{suzuki2010sufficient}, where extrapolating for the case of feature selection is natural. To perform the selection, we assume that the sufficient features are the same for the source and target domains\footnote{We discuss the situation where this might not be reasonable and propose a solution in the Supplementary Material.} so that we can estimate mutual information with training data. Recall that the mutual information of $y$ and a random vector $\rvx'$, sampled from $Q_{\rvx',y}$, with probability density function $q_{\rvx',y}$, is given by
\begin{align}\label{eq:info}
 I(y;\rvx')&=\underset{(\rvx',y)\sim Q_{\rvx',y}}{\E} \left[\text{log }\frac{q_{\rvx',y}(\rvx',y)}{q_{\rvx'}(\rvx')q_{y}(y)} \right]
\end{align}
Theorem \ref{thm:suf2} shows the theoretical foundation of using mutual information between labels and features as a guide in a feature selection procedure:

\begin{thm}\label{thm:suf2} 
Consider a random vector $\rvx=(\rvx_1,\rvx_2)$ and a random variable $\ry$ with joint distribution $Q_{\rvx,\ry}$ and p.d.f. $q_{\rvx,\ry}$. Then $I(\ry;\rvx)\geq I(\ry;\rvx_1)$ and $I(\ry;\rvx)= I(\ry;\rvx_1)$ iff $\ry \independent \rvx | \rvx_1$.
\end{thm}


The proof can be found in the Supplementary Material. Theorem \ref{thm:suf2} tells us that if we find a subset of features $\rvx_1$ from original set $\rvx=(\rvx_1,\rvx_2)$ that $I(y;\rvx)= I(y;\rvx_1)$ holds, then working with this subset can satisfy our needs, as this set is statistically sufficient for the target variable $y$. In practice, to select a good subset of features $\rvx_1$, it can be the case that we are happy with $I(y;\rvx)> I(y;\rvx_1)$, and that will depend on how much information we are willing to retrieve in exchange for a greater number of features. 


\subsection{Practical Aspects of SDR for Feature Selection}
In the ideal situation, we would like to fix a minimum acceptable value for the mutual information and try every combination of features. We thus choose the smallest subset which has enough mutual information with the target variable. Notice that the number of possible subsets $\rvx'$ of size $d'$, with $1\leq d'< d$ and $d$ being the size of the original set of features $\rvx$, is $\sum_{d'=1}^{d-1}\binom{d}{d'}=2^{d}-2$. Testing all the possibilities becomes impracticable, even if distributions that generated the data are known. We adopt a greedy strategy called \textit{SDR Forward Selection} which is an adaptation of “\textit{Forward Selection}" \cite{guyon2003introduction} with stopping rule enforcing sufficiency of selected features. At this point, we also assume that we have an estimator $\hat{I}(y;\rvx')$ for the mutual information between $y$ and a random vector $\rvx'$. We also assume that we have access to the training sample $\{(\rvx'_{i},y)\}_{i=1}^n$, independently sampled from $Q_{\rvx',y}$. We proceed by using Algorithm \ref{alg:sel} to select relevant features.
\begin{algorithm}[ht] 
\DontPrintSemicolon
 \KwIn{(i) A set of features $\mathfrak{F}=\left\{\rx^{(j)} \right\}_{j=1}^{d}$, (ii) an estimator $\hat{I}$ for mutual information between two random quantities (iii) a stopping rule that enforces sufficiency of features;}
 
 
 \KwOut{$\mathfrak{X}=\{\tilde{\rx}^{(j)}\}_{j=1}^{d'}$, that is, the subset of $d'$ features, $d'\leq d$;}


 \KwData{$\{(\rvx_{i},y_i)\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx,y}$}
 
 
 \medskip
 Initialize $j\leftarrow1$, $\mathfrak{X}\leftarrow\left\{ \right\}$ and STOP $\leftarrow$ \code{False};
 
 
 \While{\textbf{not} \textup{STOP}}
 {
 $\rx^* \leftarrow \underset{\rx \in \mathfrak{F}}{\text{argmax}} ~ \hat{I}\left(y; \mathfrak{X} \cup \{ \rx \} \right)$;
 
 
 $\mathfrak{X} \leftarrow \mathfrak{X} \cup \{ \rx^* \}$;
 
 
 $\mathfrak{F} \leftarrow \mathfrak{F} -\{ \rx^* \}$;
 
 
 \eIf{Reach the stopping rule \textbf{or} $j=d$}{
 STOP $\leftarrow$ \code{True}\;
 }{
 $j=j+1$\;
 }
 }
 \textbf{return} $\mathfrak{X}$.
\caption{SDR Forward (Feature) Selection}
\label{alg:sel}
\end{algorithm}

In other words, we start by choosing the feature that has the largest estimated mutual information with the target variable, and, at each subsequent step, we select the feature that marginally maximizes the estimated mutual information. We repeat the process until we reach a stop criterion. One example of stopping criterion that could be used when selecting features according to the Algorithm \ref{alg:sel} stops when $\hat{I}$'s marginal growth is low, hopefully yielding sufficiency of features.

When sufficient features are the same in the source and target domains\footnote{This statement refers to the solution we propose in the Supplementary Material.} and we value a more precise algorithm than a faster one, then we would want to use an adaptation of \textit{Backward Elimination} \cite{guyon2003introduction} that enforces sufficiency instead of \textit{SDR Forward Selection}. If we could correctly estimate mutual information and there is a subset of sufficient features, \textit{Backward Elimination} would certainly find one. On the other hand, \textit{Forward Selection} could not find a subset of sufficient features even if the same conditions hold. The lower speed of \textit{Backward Elimination} can be given when the number of eliminations surpasses the number of forward steps, i.e. only a few features are sufficient, or when estimating mutual information with more features costs more. Besides being faster, \textit{SDR Forward Selection} tends to work better when sufficient features are not the same in the source and target domains and the solution provided in the Supplementary Material is adopted. That is because there would be no need to use importance weighting in high-dimensions for mutual information estimation.

So far, we have assumed that we have an estimator for mutual information, but we have not discussed in-depth how to obtain this estimator. Suppose we want to estimate $I(\ry;\rvx')$ for a subset of features $\rvx'$ having a sample $\{(\rvx'_{i},\ry_i)\}_{i=1}^n$ independently sampled from $Q_{\rvx',\ry}$ with p.d.f. $q_{\rvx',\ry}$. In the next section, we present an efficient alternative for estimating mutual information to perform feature selection using finite samples, which is the use of gaussian mixture models (GMMs) \cite{reynolds2009gaussian}. 

Even though we present the following alternative for feature selection, we acknowledge that other options for mutual information estimation would fit our methodology. We choose to present the GMM option in this paper because GMMs are an efficient and well-performing alternative for feature selection through mutual information estimation for both regression \cite{eirola2014variable} and classification tasks \cite{lan2006estimating}.

%In the first option, we separately estimate the functions $\hat{q}_{\rvx',\ry}$, $\hat{q}_{\rvx'}$ and $\hat{q}_{\ry}$, and then we calculate $\hat{I}(\ry;\rvx')=n^{-1}\sum^{n}_{i=1} \text{log}[ \hat{q}_{\rvx',\ry}(\rvx'_{i},\ry_i)/(\hat{q}_{\rvx'}(\rvx_{i})\hat{q}_{\ry}(\ry_i))]$. In the second option, we directly estimate the density-ratio $ v $ and calculate $\hat{I}(\ry;\rvx')=n^{-1}\sum^{n}_{i=1} \text{log } \hat{v}(\rvx'_{i},\ry_i)$. The second option, at first, may seem more promising, given that the most common techniques for density estimation, i.e. Kernel Density Estimators, suffer from the curse of dimensionality \cite{wasserman2006all, sugiyama2012machine}, which would become a limiting factor working with many features. However, even the second option can be limiting, being an inefficient alternative since we would have to adjust a model for every subset of the tested features. 

\subsection{Gaussian Mixture Models (GMMs) for Mutual Information Estimation and Feature Selection}

If both $\ry$ and $\rvx'$ are quantitative, then we can model $\hat{q}_{\rvx',\ry}$ directly as a gaussian mixture model \cite{eirola2014variable}. In consequence, any marginal distribution of $\hat{q}_{\rvx',\ry}$, including $\hat{q}_{\rvx'}$ and $\hat{q}_{\ry}$, will be a gaussian mixture model and there is no need to fit the model more than once. If it is the case that the target variable is categorical, i.e. $y \in \{0,1,...,C-1\}$, and $\rvx'$ is quantitative, then for each value of $\ry$, we will fit a different GMM $\hat{q}_{\rvx'|\ry}(.|\ry=y)$ \cite{lan2006estimating}. In this case, we can write $\hat{q}_{\rvx',\ry}(\vx,y)= \widehat{\Prob}(\ry=y)\cdot \hat{q}_{\rvx'}(\vx|\ry=y)$, where $\widehat{\Prob}(\ry=y)$ is the empirical distribution of $\ry$. 

We have used Scikit-Learn \cite{pedregosa2011scikit} to fit GMMs and our own implementation\footnote{We have released a Python package at \url{https://github.com/felipemaiapolo/infoselect}.} to estimate the mutual information and select features. Scikit-Learn implementation for GMMs uses the EM algorithm \cite{hastie2009elements} to estimate means, covariance matrices, and the mixture parameters. The number of parameters for the standard GMM grows rapidly with problem dimensionality, we thus suggest using the alternative approaches proposed in \cite{bouveyron2007high} or \cite{tipping1999mixtures}.

==> red_dim_antigo1.tex <==
\section{The use of dimensionality reduction/feature selection to make effective sample size bigger}\label{sec:dim_red}


In this section, we present dimensionality reduction and feature selection as ways to obtain a bigger effective sample size. The two main results of this section are given by Theorems \ref{thm:div3} and \ref{thm:div4}. We show that linear dimensionality reduction and feature selection, under some conditions, decrease Rényi divergence between the target and source probability distributions, leading to a bigger effective sample size. This result accounts for the dimensionality reduction or feature selection's randomness; that is, the transformation can depend on data in some specific ways. 

To arrive at our main results, we first show the intermediate result given by Lemma \ref{lem:div2}. In the following result, $\mA$ represents a constant dimensionality reduction matrix and the vector $\vb$ represents a translation in data before dimensionality reduction, which is common when performing principal components analysis (PCA) \cite{hastie2009elements}, for example. When there is no need for considering a translation, we just can adopt $\vb=\mathbf{0}$. Also, $\mA$ can represent a feature selector, as we explain in the coming paragraphs.

\begin{lem}\label{lem:div2}
Consider (i) two absolutely continuous random vectors $\rvx \sim Q_\rvx$  and  $\rvx' \sim P_\rvx$ of size $d\geq2$, $D_2(P_{\rvx} || Q_{\rvx})<\infty$, (ii) a nonrandom constant vector $\vb \in \R^d$, and (iii) a nonrandom constant matrix $\mA \in \R^{d' \times d}$ with rank $d'$ (and $d' \leq d$). Suppose $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume $\mA (\rvx-\vb) \sim Q_{\mA (\rvx-\vb)}$ and $\mA (\rvx'-\vb) \sim P_{\mA (\rvx-\vb)}$. Then 
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\mA(\rvx-\vb)} || Q_{\mA(\rvx-\vb)})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\mA(\rvx-\vb)},Q_{\mA(\rvx-\vb)}) \geq \textup{ESS}^*(P_{\rvx},Q_{\rvx})
\end{align}
\end{lem}

The proof can be found in the appendix. 

Although Lemma \ref{lem:div2} gives us a way out in cases which the dimensionality reduction is not random, this case is not realistic. We know that, in practice, $ \mA $ and $ \vb $ are obtained using data. Theorem \ref{thm:div3} loosens the assumption that dimensionality reduction is a deterministic process.

In the next results, linear dimensionality reduction and feature selection are represented by the random matrix $ \rmA $. If we assume in advance that $ \rmA $ is absolutely continuous, then it represents an ordinary dimensionality reduction matrix. On the other hand, if $ \rmA $ is composed of zeros except for a single entry in each of its columns, which is given by one, then it represents a feature selector. Also, we can consider a random data translator $\rvb$ instead of the deterministic $\vb$.

\begin{thm}[Linear dimensionality reduction]\label{thm:div3}\linebreak 
Firstly, consider the training random samples of absolutely continuous vectors $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$ and an absolutely continuous random vector from target domain $\rvx' \sim P_{\rvx}$. Assume $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume that $D_2(P_{\rvx} || Q_{\rvx})<\infty$. Secondly, consider an absolutely continuous random vector $\rvb \in \R^{d}$ and an absolutely continuous random matrix $\rmA \in \R^{d' \times d}$, rank$(\mA)=d'$, jointly distributed according to the p.d.f. $p_{\rvb, \rmA}$, such that $(\rvb,\rmA), \rvx_i,$ and $\rvx'$ are pairwise independent, for every $i \in [n]$. Assume that $d' \leq d$. Suppose $\rmA(\rvx_i-\rvb) \sim Q_{\rmA(\rvx-\rvb)}$ and $\rmA(\rvx'-\rvb) \sim P_{\rmA(\rvx-\rvb)}$, for every $i \in [n]$, then 
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rmA (\rvx-\rvb)} || Q_{\rmA(\rvx-\rvb)})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\rmA(\rvx-\rvb)},Q_{\rmA(\rvx-\rvb)}) \geq \textup{ESS}^*(P_{\rvx},Q_{\rvx})
\end{align}
\end{thm}

The proof can be found in the appendix. 

Theorem \ref{thm:div3} tells us that a dimensionality reduction procedure before performing covariate shift adaptation increases the population effective sample size. It is important to state that Theorem \ref{thm:div3} also holds when disconsidering $\rvb$ and the proof's adaptation is straightforward. In that case, we would have that $D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rmA\rvx} || Q_{\rmA\rvx})$ and $\textup{ESS}^*(P_{\rmA\rvx},Q_{\rmA\rvx}) \geq\textup{ESS}^*(P_{\rvx},Q_{\rvx})$.

Next, in Theorem \ref{thm:div4}, we state a result regarding feature selection.

\begin{thm}[Feature selection]\label{thm:div4}\linebreak 
Firstly, consider the training random samples of absolutely continuous vectors $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$ and an absolutely continuous random vector from target domain $\rvx' \sim P_{\rvx}$. Assume $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume that $D_2(P_{\rvx} || Q_{\rvx})<\infty$. Secondly, consider a discrete random matrix $\rmA \in \R^{d' \times d}$, that represents a feature selector with rank$(\mA)=d'$, distributed according to the p.m.f. $p_{\rmA}$, such that $\rmA, \rvx_i,$ and $\rvx'$ are pairwise independent, for every $i \in [n]$. Assume that $d' \leq d$. Suppose $\rmA\rvx_i \sim Q_{\rmA\rvx}$ and $\rmA\rvx' \sim P_{\rmA\rvx}$, for every $i \in [n]$, then 
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rmA\rvx} || Q_{\rmA\rvx})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\rmA\rvx},Q_{\rmA\rvx}) \geq \textup{ESS}^*(P_{\rvx},Q_{\rvx})
\end{align}
\end{thm}

The proof can be found in the appendix. 

Theorems \ref{thm:div3} and  \ref{thm:div4} hold when the data used to obtain $\rmA$ and $\rvb$ do not depend on training data or data points that represent the target domain. That does not mean we cannot use some portion of training samples or data from the target domain to obtain $\rmA$ and $\rvb$, but it only means the results are not valid for those specific used data points. 

We now take the opportunity to present an extension of Theorem \ref{thm:div3} for nonlinear dimensionality reduction using feedforward neural networks, e.g., autoencoders. The Corollary \ref{cor:div5} presents this result:

\begin{cor}[Nonlinear dimensionality reduction]\label{cor:div5}
\linebreak 
Firstly, consider the training random samples of absolutely continuous vectors $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$ and an absolutely continuous random vector from target domain $\rvx' \sim P_{\rvx}$. Assume $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume that $D_2(P_{\rvx} || Q_{\rvx})<\infty$. Secondly, consider a feedforward neural network \linebreak$\rvh^{(K)}:\R^{d}\rightarrow \R^{d'}$ with $K-1$ hidden layers, such that 
\begin{align}
 &\rvh^{(K)}(\vx)=\\[.5em]
 &=g^{(K)}\Bigg(\rmW^{(K)} \cdots g^{(1)}\left(\rmW^{(1)} \vx +\rvb^{(1)}\right)\cdots +\rvb^{(K)}\Bigg)
\end{align}

Where $g^{(k)}$ is an invertible and differentiable activation function (e.g., sigmoid, tanh), and $\rvb^{(k)} \in \R^{d}$ and $\rmW^{(k)} \in \R^{d_k' \times d_k}$, $d_k' \leq d_k$, rank$(\rmW^{(k)})=d_k'$ are absolutely continuous random quantities jointly distributed according to the p.d.f. $p^{(k)}$. Also, consider that $(\rvb^{(k)}, \rmW^{(k)})$, $\rvx_i,$ and $\rvx'$ are pairwise independent, for every $k \in [K]$ and $i \in [n]$. Then
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rvh^{(K)}(\rvx)} || Q_{\rvh^{(K)}(\rvx)})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\rvh^{(K)}(\rvx)}, Q_{\rvh^{(K)}(\rvx)}) \geq \textup{ESS}^*(P_\rvx, Q_\rvx)
\end{align}
\end{cor}

The proof of the corollary can be found in the appendix.

Before closing this section, it is worth mentioning two points. Firstly, at the same time dimensionality reduction/feature selection solve the problem of low effective sample sizes, it might impose other problems. For example, when performing principal components analysis (PCA) \cite{hastie2009elements} for dimensionality reduction, it is not guaranteed the method will not discard useful information for the supervised task. Also, it is not even possible to ensure the covariate shift main assumption, that the conditional distribution of the labels are the same in source and target domains, still holds. In this direction, \citet{stojanov2019low} offers a clever solution to overcome these specific problems, applying sufficient dimension reduction (SDR), which is a supervised method, to reduce dimensions. Secondly, given that $\rmA$ and $\rvb$ are random quantities\footnote{This is not true when $\rmA$ and $\rvb$ are fixed.}, $\{\rmA(\rvx_i-\rvb)\}_{i=1}^n$ or $\{\rmA\rvx_i\}_{i=1}^n$ may not form independent samples, even when $\rvx_i \independent (\rmA,\rvb), \forall i \in [n]$, and $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$. If samples are not independent, then the results presented in Section \ref{sec:ess} might not hold. Unfortunately, giving the solution of this problem is not within the scope of the present paper and might be treated in future work. 

%However, this situation may not be a problem in real situations, because once we see the dataset, we can use a portion of the data to estimate $\rmA$ and then maintain it fixed, even when we receive more data points. 

%Pensar melhor no ultimo However

%Consequently, by Theorem \ref{thm:gen1}, we have that supervised methods tend to have better generalization.

==> red_dim_antigo2.tex <==
\section{The use of dimensionality reduction/feature selection to make effective sample size bigger}\label{sec:dim_red}

%Tirar primeiro teorema e mudar o segundo, incluindo bias
%Incluir experimento pca


In this section, we present dimensionality reduction and feature selection as ways to obtain a bigger effective sample size. The two main results of this section are given by Theorems \ref{thm:div2} and \ref{thm:div3}. We show that linear dimensionality reduction and feature selection, under some conditions, decrease Rényi divergence between the target and source probability distributions, leading to a bigger effective sample size. This result accounts for the dimensionality reduction or feature selection's randomness; that is, the transformation can depend on data in some specific ways. Despite Theorem \ref{thm:div2} accounting for a more general case, we think Theorem \ref{thm:div3} might be more important for practitioners, since it reflects a more concrete situation. 

In the next results, linear dimensionality reduction and feature selection are represented by the random matrix $ \rmA $. If we assume in advance that $ \rmA $ is absolutely continuous, then it represents an ordinary dimensionality reduction matrix. On the other hand, if $ \rmA $ is composed of zeros except for a single entry in each of its columns, which is given by one, then it represents a feature selector.

\begin{thm}[Linear dimensionality reduction \linebreak and feature selection]\label{thm:div2}\linebreak 
Firstly, consider the training random samples of vectors $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$ and a random vector from target domain $\rvx' \sim P_{\rvx}$. Assume $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume that $D_2(P_{\rvx} || Q_{\rvx})<\infty$. Secondly, consider an absolutely continuous or discrete random matrix $\rmA$ with distribution over $\R^{d' \times d}$, such that $(\rmA|\rvx_i=\vx)\overset{\text{dist}}{=}(\rmA|\rvx'=\vx)$, for every $i \in [n]$ and $\vx\in\sX$. Assume that $d' < d$. Suppose $\rmA\rvx_i \sim Q_{\rmA\rvx}$ and $\rmA\rvx' \sim P_{\rmA\rvx}$, for every $i \in [n]$, then 
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rmA \rvx} || Q_{\rmA \rvx})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\rmA \rvx},Q_{\rmA \rvx}) \geq \textup{ESS}^*(P_{\rvx},Q_{\rvx})
\end{align}
\end{thm}

Theorem \ref{thm:div2} tells us that a dimensionality reduction or feature selection procedure before performing covariate shift adaptation decreases the divergence between domains and increases the effective sample size if the conditional distribution of the matrix $\rmA$ given a data point from the source distribution $ Q_{\rvx}$ equals the conditional distribution of the matrix $\rmA$ given a data point from the target distribution $P_{\rvx}$. On the other hand, Theorem \ref{thm:div2} does not guarantee that the marginal distribution of $\rmA\rvx_i \sim Q_{\rmA\rvx}$ approximates the distributions of an unseen data point $\rmA\rvx''$ from the target domain, such that $\rvx'' \independent \rmA$. 

In order to overcome those difficulties, we present Theorem \ref{thm:div3}. Despite being a more specific result, deriving from the last theorem, we are able to obtain some desirable properties when narrowing the conditions. Two of them are: (i) the new conditions guarantee domains are always less divergent, even when considering unseen data, and (ii) they enable us to work in a more concrete scenario, making it easier to understand when the result's sufficient conditions hold. Essentially, Theorem \ref{thm:div3} holds when the data used to obtain $\rmA$ does not depend on training data neither on data points that represent represent the target domain. That does not mean we cannot use some portion of training samples or data from the target domain to obtain $\rmA$, but it only means the result is not valid for those specific used data points. 

\begin{thm}[Independent linear dimensionality reduction and feature selection]\label{thm:div3}\linebreak 
Firstly, consider the training random samples of vectors $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$ and a random vector from target domain $\rvx' \sim P_{\rvx}$. Assume $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume that $D_2(P_{\rvx} || Q_{\rvx})<\infty$. Secondly, consider an absolutely continuous or discrete random matrix $\rmA$ with distribution over $\R^{d' \times d}$, such that $\rmA \independent (\rvx_i,\rvx')$, for every $i \in [n]$. Assume that $d' < d$. Thirdly, consider. Suppose $\rmA\rvx_i \sim Q_{\rmA\rvx}$ and $\rmA\rvx' \sim P_{\rmA\rvx}$, for every $i \in [n]$, then 
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rmA \rvx} || Q_{\rmA \rvx})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\rmA \rvx},Q_{\rmA \rvx}) \geq \textup{ESS}^*(P_{\rvx},Q_{\rvx})
\end{align}
\begin{proof}
The proof is straightforward from Theorem \ref{thm:div2} considering that $\rmA \independent (\rvx_i,\rvx') \Rightarrow (\rmA|\rvx_i=\vx)\overset{\text{dist}}{=}(\rmA|\rvx'=\vx), \forall x \in \sX$.
\end{proof}
\end{thm}

We now take the opportunity to present an extension of Theorem \ref{thm:div2} for nonlinear dimensionality reduction using feedforward neural networks, e.g., autoencoders. The Corollary \ref{cor:div4} presents this result:

\begin{cor}[Nonlinear dimensionality reduction]\label{cor:div4}
\linebreak 
Firstly, consider the training random samples of vectors $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$ and a random vector from target domain $\rvx' \sim P_{\rvx}$. Assume $Q_{\rvx}$ and $P_{\rvx}$ measure events in $\sX \subseteq \R^d$, $d\geq2$, and have probability density functions $q_{\rvx}$ and $p_{\rvx}$, such that $\text{support}(p_{\rvx}) \subseteq \text{support}(q_{\rvx})$. Also, assume that $D_2(P_{\rvx} || Q_{\rvx})<\infty$. Secondly, consider a feedforward neural network \linebreak$\rvh^{(K)}:\R^{d}\rightarrow \R^{d'}$ with $n-1$ hidden layers, such that 
\begin{align}
 &\rvh^{(K)}(\vx)=\\[.5em]
 &=g^{(K)}\Bigg(\rmW^{(K)} \cdots g^{(2)}\bigg(\rmW^{(2)}g^{(1)}\left(\rmW^{(1)} \vx \right)\bigg)\cdots \Bigg)
\end{align}

Where $g^{(k)}$ is an invertible and differentiable activation function (e.g., sigmoid, tanh) and $\rmW^{(k)} \in \R^{d_k' \times d_k}$, $d_k' < d_k$, is an absolutely continuous or discrete random matrix, such that $(\rmW^{(k)}|\rvx_i=\vx)\overset{\text{dist}}{=}(\rmW^{(k)}|\rvx'=\vx)$, for every $k \in [K],~i \in [n] ,$ and $\vx\in\sX$. Then
\begin{align}
D_2(P_{\rvx} || Q_{\rvx})  \geq  D_2(P_{\rvh^{(K)}(\rvx)} || Q_{\rvh^{(K)}(\rvy)})
\end{align}
And, consequently,
\begin{align}
 \textup{ESS}^*(P_{\rvh^{(K)}(\rvx)}, Q_{\rvh^{(K)}(\rvy)}) \geq \textup{ESS}^*(P_\rvx, Q_\rvy)
\end{align}
\end{cor}

The proof of the corollary can be found in the appendix.

Before closing this section, it is worth to mention two points. Firstly, at the same time dimensionality reduction/feature selection solve the problem of low effective sample sizes, it might impose other problems. For example, when performing principal components analysis (PCA) \cite{hastie2009elements} for dimensionality reduction, it is not guaranteed the method will not discard useful information for the supervised task. Also, it is not even possible to ensure the covariate shift main assumption, that the conditional distribution of the labels are the same in source and target domains, still holds. In this direction, \citet{stojanov2019low} offers a clever solution to overcome these specific problems, applying sufficient dimension reduction (SDR), which is a supervised method, to reduce dimensions. Secondly, given that $\rmA$ is a random quantity, $\{\rmA\rvx_i\}_{i=1}^n$ might not form an independent sample, even when $\rvx_i \independent \rmA$ and $\{\rvx_i\}_{i=1}^n \overset{iid}{\sim} Q_{\rvx}$. If samples are not independent, then the results presented in Section \ref{sec:ess} might not hold. However, this situation may not be a problem in real situations, because once we see the dataset, we can use a portion of the data to estimate $\rmA$ and then maintain it fixed, even when we receive more data points. 





==> red_dim_antigo3.tex <==
\section{The use of dimensionality reduction/feature selection to make effective sample size bigger}\label{sec:dim_red}


In this section, we present dimensionality reduction and feature selection as ways to obtain a bigger effective sample size. The main result of this section is given by Theorem \ref{thm:div3}. We show that linear dimensionality reduction and feature selection decrease Rényi divergence between the target and source probability differences, leading to a bigger effective sample size. This result accounts for the dimensionality reduction's randomness; that is, the transformation can depend on the training data.

To arrive at our main result, we first show the intermediate result given by Lemma \ref{lem:div2}:

\begin{lem}\label{lem:div2}
Consider (i) two absolutely continuous random vectors $\rvx \sim P_\rvx$ and $\rvy \sim Q_\rvy$ of size $d\geq2$, $D_2(P_{\rvx} || Q_{\rvy})<\infty$, and (ii) a nonrandom constant matrix $\mA \in \R^{d' \times d}$ with rank $d'$ (and $d' < d$). Suppose the density function of measure $P_\rvx$ has its support contained in $Q_\rvy$ density's support, $\mA \rvx \sim P_{\mA \rvx}$, and $\mA \rvy \sim Q_{\mA \rvy}$. Then 
\begin{align}
 \textup{ESS}^*(P_{\mA \rvx},Q_{\mA \rvy}) \geq \textup{ESS}^*(P_\rvx,Q_\rvy)
\end{align}
\end{lem}

The proof can be found in the appendix. 

Although Lemma \ref{lem:div2} gives us a way out in cases where the dimensionality reduction is not random, this case is not realistic. We know that in practice, the $ \mA $ matrix is obtained using training data and methods such as Principal Component Analysis (PCA) \cite{hastie2009elements} or Sufficient Dimension Reduction (SDR) \cite{suzuki2010sufficient}. Theorem \ref{thm:div3} loosens the assumption that dimensionality reduction is a deterministic process.

\begin{thm}[Linear dimensionality reduction \linebreak and feature selection]\label{thm:div3}
Consider (i) two absolutely continuous random vectors $\rvx \sim P_{\rvx}$ and $\rvy \sim Q_{\rvy}$ of size $d\geq2$ and (ii) an absolutely continuous random matrix $\rmA$ with distribution $F$ over $\R^{d' \times d}$. Also, consider that $\rmA$ can depend on $\rvx$ or $\rvy$. Suppose that $d' < d$ and rank$(\rmA)=d'$. Suppose $\rmA \rvx \sim P_{\mA \rvx}$ and $\rmA \rvy \sim Q_{\mA \rvy}$. Then 
\begin{align}
 \textup{ESS}^*(P_{\mA \rvx},Q_{\mA \rvy}) \geq \textup{ESS}^*(P_\rvx,Q_\rvy)
\end{align}
Remark: If we assume in advance that $ \rmA $ is composed of zeros except for a single entry in each of its columns, which is given by one, then we have the case of feature selection. That is, feature selection is a special case of dimensionality reduction. In this case, $ \rmA $ would have a discrete distribution; consequently, the appendix's proof would have to be adapted. That adaptation is straightforward.
\end{thm}

The proof can be found in the appendix. 

Theorem \ref{thm:div3} tells us that a dimensionality reduction or feature selection procedure before performing covariate shift adaptation increases the population effective sample size. Consequently, by Theorem \ref{thm:gen1}, we have that supervised methods tend to have better generalization. To close this section, we take the opportunity to present an extension of Theorem \ref {thm:div3} for nonlinear dimensionality reduction using feedforward neural networks, e.g., autoencoders. The Corollary \ref{cor:div4} presents this result:

\begin{cor}[Nonlinear dimensionality reduction]\label{cor:div4}
\linebreak Consider a feedforward neural network \linebreak$\rvh^{(n)}:\R^{d}\rightarrow \R^{d'}$ with $n-1$ hidden layers, such that 
\begin{align}
 &\rvh^{(n)}(\vx)=\\[.5em]
 &=g^{(n)}\Bigg(\rmW^{(n)} \cdots g^{(2)}\bigg(\rmW^{(2)}g^{(1)}\left(\rmW^{(1)} \vx \right)\bigg)\cdots \Bigg)
\end{align}

Where $g^{(j)}$ is an invertible and differentiable activation function (e.g., sigmoid, tanh) and $\rmW^{(j)} \in \R^{d_j' \times d_j}$ is a random matrix, being true that $d_j' < d_j$ and rank$(\rmW^{(j)})=d_j'$. Then, if $\rvx \sim P_\rvx$ and $\rvy \sim Q_\rvy$ we have that
\begin{align}
 \textup{ESS}^*(P_{\rvh^{(n)}(\rvx)}, Q_{\rvh^{(n)}(\rvy)}) \geq \textup{ESS}^*(P_\rvx, Q_\rvy)
\end{align}
\end{cor}

The proof of the corollary can be found in the appendix.

In Section \ref{sec:exp}, we present regression and classification experiments in which we perform feature selection before covariate shift adaptation. Through our experiments, we were able to verify that the feature selection stage tends to increase the effective sample size, consequently allowing better performance of supervised methods.

==> supp_antigo1.tex <==
\onecolumn
\section{Appendix}

\subsection{Proofs and Derivations}

\subsubsection{Proof of Theorem \ref{thm:ess}}
\begin{proof}
Assume the hypothesis stated are valid. Being $c\neq 0$ a real constant, see we can re-wright the ESS as follows:
\begin{align*}
 \widehat{\textup{ESS}}_n(P_\rvx, Q_\rvx)&=\frac{(\sum_{i=1}^n \rw_i)^2}{n\sum_{i=1}^n \rw_i^2}=\frac{\left[\sum_{i=1}^n c\cdot \frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}{n\sum_{i=1}^n  \left[c\cdot \frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}=\frac{\left[\frac{1}{n}\sum_{i=1}^n  \frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}{\frac{1}{n}\sum_{i=1}^n  \left[\frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}\\[.5em]
\end{align*}

Then, by the Strong Law of Large Numbers and almost-sure convergence properties \cite{roussas1997course}, we verify that $\widehat{\textup{ESS}}_n(P_\rvx, Q_\rvx) \xrightarrow[]{a.s.} \frac{\E_{\rvx \sim Q_\rvx}\left[\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)} \right]^2}{\E_{\rvx \sim Q_\rvx}\left[\left(\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)}\right)^2 \right]} \text{ when } n \rightarrow \infty$. To complete the proof, we state the following
\begin{align*}
 \frac{\E_{\rvx \sim Q_\rvx}\left[\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)} \right]^2}{\E_{\rvx \sim Q_\rvx}\left[\left(\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)}\right)^2 \right]} &=\frac{1}{\E_{\rvx \sim P_\rvx}\left[\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)} \right]}=\frac{1}{\textup{exp}\left[D_2(P_\rvx || Q_\rvx)\right]}=\text{ESS}^*(P_\rvx, Q_\rvx)
\end{align*}
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:div1}}
\begin{proof}
Assume the hypothesis are valid and let $d_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})$ = $\text{exp}[D_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})]$. See that:
\begin{align*}
 d_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})&= \E_{P_{\rvx_1,\rvx_2}} \left[\frac{p_{\rvx_1,\rvx_2}(\rvx_1,\rvx_2)}{q_{\rvx_1,\rvx_2}(\rvx_1,\rvx_2)}\right] = \E_{P_{\rvx_1}} \left[\frac{p_{\rvx_1}(\rvx_1)}{q_{\rvx_1}(\rvx_1)}\cdot \E_{P_{\rvx_2|\rvx_1}} \left[\frac{p_{\rvx_2|\rvx_1}(\rvx_2|\rvx_1)}{q_{\rvx_2|\rvx_1}(\rvx_2|\rvx_1)}\right]\right] =\\[.5em]
 &=\E_{P_{\rvx_1}} \left[\frac{p_{\rvx_1}(\rvx_1)}{q_{\rvx_1}(\rvx_1)}\cdot d_2(P_{\rvx_2|\rvx_1} || Q_{\rvx_2|\rvx_1})\right] \geq \E_{P_{\rvx_1}}   \left[\frac{p_{\rvx_1}(\rvx_1)}{q_{\rvx_1}(\rvx_1)}\right]=d_2(P_{\rvx_1} || Q_{\rvx_1})\\[.5em]
\end{align*}

Where the inequality is obtained by the fact that the exponential of the Rényi Divergence must be greater or equals one. To complete the proof, see that $\textup{ESS}^*(P_{\rvx_1,\rvx_2}, Q_{\rvx_1,\rvx_2})=d_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})^{-1}$. Therefore
\begin{align*}
    \textup{ESS}^*(P_{\rvx_1}, Q_{\rvx_1}) \geq \textup{ESS}^*(P_{\rvx_1,\rvx_2}, Q_{\rvx_1,\rvx_2})
\end{align*}
\end{proof}

\subsubsection{Proof of Lemma \ref{lem:div2}}
\begin{proof}
If $d=d'$, the result is direct considering Theorem 1 from \citet{qiao2010study}. Otherwise, consider a full rank matrix $\mC=\begin{bmatrix}
\mA\\ 
\mB
\end{bmatrix} \in \R^{d \times d}$, where $\mB \in \R^{d-d',d}$. Given that $\mC$ is full rank, it represents a invertible linear (and differentiable) transformation. If $\mC (\rvx-\vb)=\begin{bmatrix}
\mA(\rvx-\vb)\\ 
\mB(\rvx-\vb)
\end{bmatrix} \sim Q_{\mC (\rvx-\vb)}$ and $\mC (\rvx'-\vb)=\begin{bmatrix}
\mA(\rvx'-\vb)\\ 
\mB(\rvx'-\vb)
\end{bmatrix}\sim P_{\mC (\rvx'-\vb)}$, then by Theorem 1 from \citet{qiao2010study} we have that $ D_2(P_{\rvx} || Q_{\rvx}) = D_2(P_{\mC (\rvx-\vb)} || Q_{\mC (\rvx-\vb)})$. Discarding $\mB(\rvx-\vb)$ and $\mB(\rvx'-\vb)$ from random vectors $\mC(\rvx-\vb)$ and $\mC(\rvx'-\vb)$, by Theorem \ref{thm:div1}, we have that
\begin{align*}
D_2(P_{\rvx} || Q_{\rvx}) \geq D_2(P_{\mA (\rvx-\vb)} || Q_{\mA (\rvx-\vb)})
\end{align*}

Therefore
\begin{align*}
  &\textup{ESS}^*(P_{\mA (\rvx-\vb)}, Q_{\mA (\rvx-\vb)})=\exp\left[-D_2(P_{\mA (\rvx-\vb)} || Q_{\mA (\rvx-\vb)}) \right]\geq \exp\left[-D_2(P_{\rvx} || Q_{\rvx}) \right] =\textup{ESS}^*(P_{\rvx}, Q_{\rvx})
\end{align*}
\end{proof}



\subsubsection{Proof of Theorem \ref{thm:div3}}
\begin{proof}
Firstly, we define $\rvv:=\rmA (\rvx_i-\rvb) \sim Q_{\rvv} \equiv Q_{\rmA (\rvx-\rvb)}$ and $\rvu:=\rmA (\rvx'-\rvb) \sim P_{\rvu} \equiv P_{\rmA (\rvx-\rvb)}$, for an arbitrary $i \in [n]$. Let $q_{\rvv}$ and $p_{\rvu}$ be probability density functions associated with distributions $Q_{\rvv}$ and $P_{\rvu}$. From Lemma \ref{lem:div2}, we know that  $D_2\left(P_{\rvu|\rvb=\vb,\rmA=\mA}||Q_{\rvv|\rvb=\vb,\rmA=\mA} \right) \leq D_2\left( P_{ \rvx} || Q_{ \rvx} \right), \forall\vb\in\R^d$, $\forall \mA \in \R^{d' \times d}$ such that rank$(\mA)=d'$. That statement implies the following:
\begin{align*}
  &\exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow \E_{p_{\rvb, \rmA}}\left[\exp D_2\left(P_{\rvu|\rvb,\rmA}||Q_{\rvv|\rvb,\rmA} \right)\right] \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow \int p_{\rvb, \rmA}(\vb,\mA)\int p_{\rvu|\rvb,\rmA}(\vu|\vb,\mA)\frac{p_{\rvu|\rvb,\rmA}(\vu|\vb,\mA)}{q_{\rvv|\rvb,\rmA}(\vu|\vb,\mA)}\text{d}\vu\text{d}\vb\text{d}\mA \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow \int p_{\rvu|\rvb,\rmA}(\vu|\vb,\mA)p_{\rvb, \rmA}(\vb,\mA)\frac{p_{\rvu|\rvb,\rmA}(\vu|\vb,\mA)}{q_{\rvv|\rvb,\rmA}(\vu|\vb,\mA)}\frac{p_{\rvb, \rmA}(\vb,\mA)}{p_{\rvb, \rmA}(\vb,\mA)}\text{d}\vu\text{d}\vb\text{d}\mA \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow D_2\left(P_{\rvu,\rvb,\rmA}||Q_{\rvv,\rvb,\rmA} \right) \leq D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow D_2\left(P_{\rmA (\rvx-\rvb)}||Q_{\rmA (\rvx-\rvb)} \right) = D_2\left(P_{\rvu}||Q_{\rvv} \right) \leq D_2\left(P_{\rvu,\rvb,\rmA}||Q_{\rvv,\rvb,\rmA} \right)\leq D_2\left( P_\rvx || Q_\rvx \right)\\[1em]
\end{align*}

The last step is due to the Theorem \ref{thm:div1}. To complete the proof, we state the following:
\begin{align*}
  &\textup{ESS}^*(P_{\rmA (\rvx-\rvb)}, Q_{\rmA (\rvx-\rvb)})=\exp\left[-D_2(P_{\rmA (\rvx-\rvb)} || Q_{\rmA (\rvx-\rvb)}) \right]\geq \exp\left[-D_2(P_{\rvx} || Q_{\rvx}) \right] =\textup{ESS}^*(P_{\rvx}, Q_{\rvx})
\end{align*}
\end{proof}

\subsubsection{Proof of Theorem \ref{thm:div4}}
\begin{proof}
Firstly, we define $\rvv:=\rmA \rvx_i \sim Q_{\rvv} \equiv Q_{\rmA \rvx}$ and $\rvu:=\rmA \rvx' \sim P_{\rvu} \equiv P_{\rmA \rvx}$, for an arbitrary $i \in [n]$. Let $q_{\rvv}$ and $p_{\rvu}$ be probability density functions associated with distributions $Q_{\rvv}$ and $P_{\rvu}$. From Lemma \ref{lem:div2}, we know that  $D_2\left(P_{\rvu|\rmA=\mA}||Q_{\rvv|\rmA=\mA} \right) \leq D_2\left( P_{ \rvx} || Q_{ \rvx} \right)$, $\forall \mA \in \R^{d' \times d}$ such that rank$(\mA)=d'$. That statement implies the following:

\begin{align*}
  &D_2\left(P_{\rvu|\rmA=\mA}||Q_{\rvv|\rmA=\mA} \right) \leq D_2\left( P_{\rvx} || Q_{\rvy} \right)\Rightarrow \exp D_2\left(P_{\rvu|\rmA=\mA}||Q_{\rvv|\rmA=\mA} \right) \leq \exp D_2\left( P_\rvx || Q_\rvy \right)\Rightarrow\\[1em]
  &\Rightarrow \E_{p_\rmA}\left[\exp D_2\left(P_{\rvu|\rmA}||Q_{\rvv|\rmA} \right)\right] \leq \exp D_2\left( P_\rvx || Q_\rvy \right)\Rightarrow \sum_{\mA} p_\rmA(\mA)\int p_{\rvu|\rmA}(\vu|\mA)\frac{p_{\rvu|\rmA}(\vu|\mA)}{q_{\rvv|\rmA}(\vu|\mA)}\text{d}\vu \leq \exp D_2\left( P_\rvx || Q_\rvy \right)\Rightarrow\\[1em]
  &\Rightarrow \sum_{\mA} \int  p_{\rvu|\rmA}(\vu|\mA)p_\rmA(\mA)\frac{p_{\rvu|\rmA}(\vu|\mA)}{q_{\rvv|\rmA}(\vu|\mA)}\frac{p_\rmA(\mA)}{p_\rmA(\mA)}\text{d}\vu \leq \exp D_2\left( P_\rvx || Q_\rvy \right)\Rightarrow D_2\left(P_{\rvu,\rmA}||Q_{\rvv,\rmA} \right) \leq D_2\left( P_\rvx || Q_\rvy \right)\Rightarrow\\[1em]
  &\Rightarrow D_2\left(P_{\rmA \rvx}||Q_{\rmA \rvy} \right) = D_2\left(P_{\rvu}||Q_{\rvv} \right) \leq D_2\left(P_{\rvu,\rmA}||Q_{\rvv,\rmA} \right)\leq D_2\left( P_\rvx || Q_\rvy \right)\\[1em]
\end{align*}

Where the sum is given over a finite number of values of $\mA$. The last step is due to the Theorem \ref{thm:div1}. To complete the proof, we state the following:
\begin{align*}
  &\textup{ESS}^*(P_{\rmA \rvx}, Q_{\rmA \rvy})=\exp\left[-D_2(P_{\rmA \rvx} || Q_{\rmA \rvy}) \right]\geq \exp\left[-D_2(P_{\rvx} || Q_{\rvx}) \right] =\textup{ESS}^*(P_{\rvx}, Q_{\rvy})
\end{align*}
\end{proof}

\subsubsection{Proof of Corollary \ref{cor:div5}}
\begin{proof}

%\equiv Q_{g^{(k)}(\rmW^{(k)} \rvh^{(k-1)}(\rvx_i) + \rvb^{(k)})}
% \equiv P_{g^{(k)}(\rmW^{(k)} \rvh^{(k-1)}(\rvx') + \rvb^{(k)})}

Firstly, we define $\rvh^{(k)}(\rvx_i):=g^{(k)}(\rmW^{(k)} \rvh^{(k-1)}(\rvx_i) + \rvb^{(k)}) \sim Q_{\rvh^{(k)}(\rvx_i)}$ and $\rvh^{(k)}(\rvx'):=g^{(k)}(\rmW^{(k)} \rvh^{(k-1)}(\rvx') + \rvb^{(k)})\sim P_{\rvh^{(k)}(\rvx')}$, for arbitrary $i \in [n]$ and $k \in [K]$. Let $q_{\rvh^{(k)}(\rvx_i)}$ and $p_{\rvh^{(k)}(\rvx')}$ be probability density functions associated with distributions $Q_{\rvh^{(k)}(\rvx_i)}$ and $P_{\rvh^{(k)}(\rvx')}$. From Lemma \ref{lem:div2} and Theorem 1 of \citet{qiao2010study}, we know that  $D_2\left(P_{\rvh^{(k)}(\rvx')|\rmW^{(k)}=\mW, \rvb^{(k)}=\vb}||Q_{\rvh^{(k)}(\rvx_i)|\rmW^{(k)}=\mW, \rvb^{(k)}=\vb} \right) \leq D_2\left(P_{\rvh^{(k-1)}(\rvx')} || Q_{\rvh^{(k-1)}(\rvx'_1)} \right)$, $\forall \mW \in \R^{d'_k \times d_k}$ and $\forall \vb \in \R^{d'_k}$ such that rank$(\mW)=d'_k$. That statement implies the following:
\begin{align*}
  &D_2\left(P_{\rvh^{(k)}(\rvx')|\rmW^{(k)}=\mW, \rvb^{(k)}=\vb}||Q_{\rvh^{(k)}(\rvx_i)|\rmW^{(k)}=\mW, \rvb^{(k)}=\vb} \right) \leq D_2\left( P_{\rvx} || Q_{\rvx} \right)\Rightarrow\\[1em]
  &\Rightarrow \exp D_2\left(P_{\rvh^{(k)}(\rvx')|\rmW^{(k)}=\mW, \rvb^{(k)}=\vb}||Q_{\rvh^{(k)}(\rvx_i)|\rmW^{(k)}=\mW, \rvb^{(k)}=\vb} \right) \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow \E_{p^{(k)}}\left[\exp D_2\left(P_{\rvh^{(k)}(\rvx')|\rmW^{(k)}, \rvb^{(k)}}||Q_{\rvh^{(k)}(\rvx_i)|\rmW^{(k)}, \rvb^{(k)}} \right)\right] \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow \int p^{(k)}(\mW,\vb)\int p_{\rvh^{(k)}(\rvx')|\rmW^{(k)}, \rvb^{(k)}}(\vu|\mW,\vb)\frac{p_{\rvh^{(k)}(\rvx')|\rmW^{(k)}, \rvb^{(k)}}(\vu|\mW,\vb)}{q_{\rvh^{(k)}(\rvx_i)|\rmW^{(k)}, \rvb^{(k)}}(\vu|\mW,\vb)}\text{d}\vu\text{d}\mW\text{d}\vb \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow \int p_{\rvh^{(k)}(\rvx')|\rmW^{(k)}, \rvb^{(k)}}(\vu|\mW,\vb)p^{(k)}(\mW,\vb)\frac{p_{\rvh^{(k)}(\rvx')|\rmW^{(k)}, \rvb^{(k)}}(\vu|\mW,\vb)}{q_{\rvh^{(k)}(\rvx_i)|\rmW^{(k)}, \rvb^{(k)}}(\vu|\mW,\vb)}\frac{p^{(k)}(\mW,\vb)}{p^{(k)}(\mW,\vb)}\text{d}\vu\text{d}\mW\text{d}\vb \leq \exp D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow D_2\left(P_{\rvh^{(k)}(\rvx'),\rmW^{(k)}, \rvb^{(k)}}||Q_{\rvh^{(k)}(\rvx_i),\rmW^{(k)}, \rvb^{(k)}} \right) \leq D_2\left( P_\rvx || Q_\rvx \right)\Rightarrow\\[1em]
  &\Rightarrow D_2\left(P_{\rmA (\rvx-\rvb)}||Q_{\rmA (\rvx-\rvb)} \right) = D_2\left(P_{\rvh^{(k)}(\rvx')}||Q_{\rvh^{(k)}(\rvx_i)} \right) \leq D_2\left(P_{\rvh^{(k)}(\rvx'),\rmW^{(k)}, \rvb^{(k)}}||Q_{\rvh^{(k)}(\rvx_i),\rmW^{(k)}, \rvb^{(k)}} \right)\leq D_2\left( P_\rvx || Q_\rvx \right)\\[1em]
\end{align*}


Firstly, see that from Lemma \ref{lem:div2}, it is true that

$\rmW^{(k)}\vx+\rvb^{(k)}=\rmW^{(k)}(\vx-\Tilde{\rvb}^{(k)})$, if $\rvb^{(k)}=-\rmW^{(k)}\Tilde{\rvb}^{(k)}$, for some random vector $\Tilde{\rvb}^{(k)}$. Secondly, note that $\rvh^{(j+1)}(\vx)=g^{(j+1)}\left(\rmW^{(j+1)}\rvh^{(j)}(\vx)+\rvb^{(j+1)}\right)$, for $j\geq0$, considering $\rvh^{(0)}(\vx)=\vx$. By Theorem \ref{thm:div2} and Theorem 1 from \citet{qiao2010study}, it is direct that
\begin{align*}
 D_2(P_{\rvh^{(j)}(\rvx)} || Q_{\rvh^{(j)}(\rvx)}) \geq D_2(P_{\rvh^{(j+1)}(\rvx)} || Q_{\rvh^{(j+1)}(\rvy)})
\end{align*}

Consequently,
\begin{align*}
  &D_2(P_\rvx || Q_\rvx)=D_2(P_{\rvh^{(0)}(\rvx)} || Q_{\rvh^{(0)}(\rvx)}) \geq D_2(P_{\rvh^{(1)}(\rvx)} || Q_{\rvh^{(1)}(\rvy)}) \geq \cdots  \geq D_2(P_{\rvh^{(n)}(\rvx)} || Q_{\rvh^{(n)}(\rvy)})
\end{align*}
To complete the proof, we state the following:
\begin{align*}
    &\textup{ESS}^*(P_{\rvh^{(n)}(\rvx)}, Q_{\rvh^{(n)}(\rvy)})=\exp\left[-D_2(P_{\rvh^{(n)}(\rvx)} || Q_{\rvh^{(n)}(\rvy)}) \right]\geq \exp\left[-D_2(P_{\rvx} || Q_{\rvx}) \right] =\textup{ESS}^*(P_{\rvx}, Q_{\rvy})
\end{align*}
\end{proof}


\subsection{Experiments}


In the experiments section, we tune three hyperparameters: (i) $l1$ regularization parameter used to train the logistic regression model when estimating $w$, (ii) the minimum number of samples per leaf in each regression/classification tree, and (iii) number of GMM components. We use the Scikit-Learn \cite{pedregosa2011scikit} implementations to train the logistic regressions, regression/classification trees and GMMs. Firstly, we choose the $l1$ logistic regression regularization parameter $C$ from values in $[10^{-4},5]$, in order to minimize the log loss in a holdout dataset. Secondly, we choose the minimum number of samples per leaf in each regression/classification tree from values in $[5,15,25,40,50]$, in order to minimize the mean squared error or classification error within a 2-fold cross-validation procedure. Finally, we maximize the log-likelihood in a holdout dataset to choose the number of GMM components, varying the possible number of components within the list $[1,...,15]$.

==> supp_antigo2.tex <==
\onecolumn
\section{Appendix}

\subsection{Proofs and Derivations}

\subsubsection{Proof of Theorem \ref{thm:ess}}
\begin{proof}
Assume the hypothesis stated are valid. Being $c\neq 0$ a real constant, see we can re-wright the ESS as follows:
\begin{align*}
 \widehat{\textup{ESS}}_n(P_\rvx, Q_\rvx)&=\frac{(\sum_{i=1}^n \rw_i)^2}{n\sum_{i=1}^n \rw_i^2}\\[.5em]
 &=\frac{\left[\sum_{i=1}^n c\cdot \frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}{n\sum_{i=1}^n  \left[c\cdot \frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}\\[.5em]
 &=\frac{\left[\frac{1}{n}\sum_{i=1}^n  \frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}{\frac{1}{n}\sum_{i=1}^n  \left[\frac{p_{\rvx}(\rvx_i)}{q_{\rvx}(\rvx_i)}\right]^2}\\[.5em]
\end{align*}

Then, by the Strong Law of Large Numbers and almost-sure convergence properties \cite{roussas1997course}, we verify that $\widehat{\textup{ESS}}_n(P_\rvx, Q_\rvx) \xrightarrow[]{a.s.} \frac{\E_{\rvx \sim Q_\rvx}\left[\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)} \right]^2}{\E_{\rvx \sim Q_\rvx}\left[\left(\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)}\right)^2 \right]} \text{ when } n \rightarrow \infty$. To complete the proof, we state the following
\begin{align*}
 \frac{\E_{\rvx \sim Q_\rvx}\left[\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)} \right]^2}{\E_{\rvx \sim Q_\rvx}\left[\left(\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)}\right)^2 \right]} &=\frac{1}{\E_{\rvx \sim P_\rvx}\left[\frac{p_\rvx(\rvx)}{q_\rvx(\rvx)} \right]}\\[.5em]
 &=\frac{1}{\textup{exp}\left[D_2(P_\rvx || Q_\rvx)\right]}\\[.5em]
 &=\text{ESS}^*(P_\rvx, Q_\rvx)
\end{align*}
\end{proof}


\subsubsection{Proof of Theorem \ref{thm:div1}}
\begin{proof}
Assume the hypothesis are valid and let\linebreak $d_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})$ = $\text{exp}[D_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})]$. See that:
\begin{align*}
 &d_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})= \\[.5em]
 &= \E_{P_{\rvx_1,\rvx_2}} \left[\frac{p_{\rvx_1,\rvx_2}(\rvx_1,\rvx_2)}{q_{\rvx_1,\rvx_2}(\rvx_1,\rvx_2)}\right] \\[.5em]
 &= \E_{P_{\rvx_1}} \left[\frac{p_{\rvx_1}(\rvx_1)}{q_{\rvx_1}(\rvx_1)}\cdot \E_{P_{\rvx_2|\rvx_1}} \left[\frac{p_{\rvx_2|\rvx_1}(\rvx_2|\rvx_1)}{q_{\rvx_2|\rvx_1}(\rvx_2|\rvx_1)}\right]\right] \\[.5em]
 &= \E_{P_{\rvx_1}} \left[\frac{p_{\rvx_1}(\rvx_1)}{q_{\rvx_1}(\rvx_1)}\cdot d_2(P_{\rvx_2|\rvx_1} || Q_{\rvx_2|\rvx_1})\right]\\[.5em]
 & \geq \E_{P_{\rvx_1}}   \left[\frac{p_{\rvx_1}(\rvx_1)}{q_{\rvx_1}(\rvx_1)}\right]=d_2(P_{\rvx_1} || Q_{\rvx_1})
\end{align*}
Where the inequality is obtained by the fact that the exponential of the Rényi Divergence must be greater or equals one. To complete the proof, see that \linebreak$\textup{ESS}^*(P_{\rvx_1,\rvx_2}, Q_{\rvx_1,\rvx_2})=d_2(P_{\rvx_1,\rvx_2} || Q_{\rvx_1,\rvx_2})^{-1}$. Therefore
\begin{align*}
    \textup{ESS}^*(P_{\rvx_1}, Q_{\rvx_1}) \geq \textup{ESS}^*(P_{\rvx_1,\rvx_2}, Q_{\rvx_1,\rvx_2})
\end{align*}
\end{proof}

\subsubsection{Proof of Theorem \ref{thm:div2}}
\begin{proof}
Firstly, we define $\rvu:=\rmA \rvx_i \sim Q_{\rvu} \equiv Q_{\rmA \rvx}$ and $\rvv:=\rmA \rvx'_j \sim P_{\rvv} \equiv P_{\rmA \rvx}$. Secondly, see that $(\rmA|\rvx_i=\vx)\overset{\text{dist}}{=}(\rmA|\rvx'_j=\vx) \Rightarrow (\rvu|\rvx_i=\vx)\overset{\text{dist}}{=}(\rvv|\rvx'_j=\vx),\forall\vx\in\sX$. Assuming $\rmA$ is absolutely continuous, let $q_{\rvu|\rvx}=p_{\rvv|\rvx}$ be probability density functions associated with distributions $Q_{\rvu|\rvx}=P_{\rvv|\rvx}$. We have the following:
\begin{align*}
    &D_2\left(P_{\rvx}||Q_{\rvx} \right)= \\[.5em]
    &=\int p_{\rvx}(\vx)\frac{p_{\rvx}(\vx)}{q_{\rvx}(\vx)}\text{d}\vx\\[.5em]
    &=\int\int p_{\rvx}(\vx)p_{\rvv|\rvx}(\vv|\vx)\frac{p_{\rvx}(\vx)}{q_{\rvx}(\vx)}\frac{p_{\rvv|\rvx}(\vv|\vx)}{p_{\rvv|\rvx}(\vv|\vx)}\text{d}\vv\text{d}\vx\\[.5em]
    &=\int\int p_{\rvx}(\vx)p_{\rvv|\rvx}(\vv|\vx)\frac{p_{\rvx}(\vx)}{q_{\rvx}(\vx)}\frac{p_{\rvv|\rvx}(\vv|\vx)}{q_{\rvu|\rvx}(\vv|\vx)}\text{d}\vv\text{d}\vx\\[.5em]
    &=D_2\left(P_{\rvx,\rvv}||Q_{\rvx,\rvu} \right) \geq  D_2\left(P_{\rvv}||Q_{\rvu} \right) = D_2\left(P_{\rmA \rvx}||Q_{\rmA \rvx} \right)
\end{align*}

The last line is is given by Theorem \ref{thm:div1}. To complete the proof, we state the following:
\begin{align*}
    &\textup{ESS}^*(P_{\rmA \rvx}, Q_{\rmA \rvy})=\exp\left[-D_2(P_{\rmA \rvx} || Q_{\rmA \rvy}) \right]\\[.5em]
    &\geq \exp\left[-D_2(P_{\rvx} || Q_{\rvx}) \right] =\textup{ESS}^*(P_{\rvx}, Q_{\rvy})
\end{align*}

If we consider $\rmA$ discrete, then there is only a need to substitute one of the integrals for a sum.
\end{proof}

\subsubsection{Proof of Corollary \ref{cor:div4}}
\begin{proof}
Firstly, see that $\rvh^{(j+1)}(\vx)=g^{(j+1)}\left(\rmW^{(j+1)}\rvh^{(j)}(\vx)\right)$, for $j\geq0$. Consider $\rvh^{(0)}(\vx)=\vx$. By Theorem \ref{thm:div2} and Theorem 1 from \citet{qiao2010study}, it is direct that
\begin{align*}
 D_2(P_{\rvh^{(j)}(\rvx)} || Q_{\rvh^{(j)}(\rvx)}) \geq D_2(P_{\rvh^{(j+1)}(\rvx)} || Q_{\rvh^{(j+1)}(\rvy)})
\end{align*}

Consequently,
\begin{align*}
  &D_2(P_\rvx || Q_\rvx)=D_2(P_{\rvh^{(0)}(\rvx)} || Q_{\rvh^{(0)}(\rvx)}) \geq \\ 
  &\geq D_2(P_{\rvh^{(1)}(\rvx)} || Q_{\rvh^{(1)}(\rvy)}) \geq \cdots  \geq D_2(P_{\rvh^{(n)}(\rvx)} || Q_{\rvh^{(n)}(\rvy)})
\end{align*}
To complete the proof, we state the following:
\begin{align*}
    &\textup{ESS}^*(P_{\rvh^{(n)}(\rvx)}, Q_{\rvh^{(n)}(\rvy)})=\exp\left[-D_2(P_{\rvh^{(n)}(\rvx)} || Q_{\rvh^{(n)}(\rvy)}) \right]\\[.5em]
    &\geq \exp\left[-D_2(P_{\rvx} || Q_{\rvx}) \right] =\textup{ESS}^*(P_{\rvx}, Q_{\rvy})
\end{align*}
\end{proof}


\subsection{Experiments}


In the experiments section, we tune three hyperparameters: (i) $l1$ regularization parameter used to train the logistic regression model when estimating $w$, (ii) the minimum number of samples per leaf in each regression/classification tree, and (iii) number of GMM components. We use the Scikit-Learn \cite{pedregosa2011scikit} implementations to train the logistic regressions, regression/classification trees and GMMs. First, we choose the $l1$ logistic regression regularization parameter $C$ from values in $[10^{-4},5]$, in order to minimize the log loss in a holdout dataset. Second, we choose the minimum number of samples per leaf in each regression/classification tree from values in $[5,15,25,40,50]$, in order to minimize the mean squared error or classification error within a 2-fold cross-validation procedure. Finally, we maximize the log-likelihood in a holdout dataset to choose the number of GMM components, varying the possible number of components within the list $[1,...,15]$.
